Generic and Robust Root Cause Localization for Multi-Dimensional Data in Online Service Systems

Localizing root causes for multi-dimensional data is critical to ensure online service systems' reliability. When a fault occurs, only the measure values within specific attribute combinations are abnormal. Such attribute combinations are substantial clues to the underlying root causes and thus are called root causes of multidimensional data. This paper proposes a generic and robust root cause localization approach for multi-dimensional data, PSqueeze. We propose a generic property of root cause for multi-dimensional data, generalized ripple effect (GRE). Based on it, we propose a novel probabilistic cluster method and a robust heuristic search method. Moreover, we identify the importance of determining external root causes and propose an effective method for the first time in literature. Our experiments on two real-world datasets with 5400 faults show that the F1-score of PSqueeze outperforms baselines by 32.89%, while the localization time is around 10 seconds across all cases. The F1-score in determining external root causes of PSqueeze achieves 0.90. Furthermore, case studies in several production systems demonstrate that PSqueeze is helpful to fault diagnosis in the real world.

==> makefile <==
TEX_FILES = $(shell find . -name '*.tex')
MAIN_TEX = main.tex
TARGET_PDF = main.pdf
CROP_FIGURE_OPERATIONS = $(shell find 'figures' -name '*.pdf' | sed -E 's/(.*)/\1.crop/g' | sed 's/ /\\ /g')

.SECONDARY:

.PHONY: crop phony_explicit build sync

build: $(TARGET_PDF);

crop: $(CROP_FIGURE_OPERATIONS);

clean:
	latexmk --output-directory=. -C

sync:
	(git add -u && git commit -m "$(date) local update") || echo nothing to commit
	git pull --no-edit
	git push


%.crop: % phony_explicit
	pdfcrop $< $<

.PHONY: build
cfl.pdf: crop $(TEX_FILES)
	bash -c 'latexmk -C; latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX)'

